GUIDE-CoT: Goal-driven and User-Informed Dynamic Estimation for Pedestrian Trajectory using Chain-of-Thought

While Large Language Models (LLMs) have recently shown impressive results in reasoning tasks, their application to pedestrian trajectory prediction remains challenging due to two key limitations: insufficient use of visual information and the difficulty of predicting entire trajectories. To address these challenges, we propose Goal-driven and User-Informed Dynamic Estimation for pedestrian trajectory using Chain-of-Thought (GUIDE-CoT). Our approach integrates two innovative modules: (1) a goal-oriented visual prompt, which enhances goal prediction accuracy combining visual prompts with a pretrained visual encoder, and (2) a chain-of-thought (CoT) LLM for trajectory generation, which generates realistic trajectories toward the predicted goal. Moreover, our method introduces controllable trajectory generation, allowing for flexible and user-guided modifications to the predicted paths. Through extensive experiments on the ETH/UCY benchmark datasets, our method achieves state-of-the-art performance, delivering both high accuracy and greater adaptability in pedestrian trajectory prediction. Our code is publicly available at https://github.com/ai-kmu/GUIDE-CoT.

==> tables/tab3.tex <==
\begin{table}
\caption{Ablation study of goal-oriented visual prompts on ETH/UCY datasets and FDE($\downarrow$) as the evaluation metric.}
\label{tab2}
{\setlength{\tabcolsep}{3.2pt}
\begin{tabular}{cc|cccccc}
\toprule
$\mathcal{X}_{\text{sem}}$ & $\mathcal{X}_{\text{vis}}$ & \textbf{ETH} & \textbf{HOTEL} & \textbf{UNIV} & \textbf{ZARA1} & \textbf{ZARA2} & \textbf{AVG} \\
\midrule
\checkmark & & 0.66 & 0.22 & 0.64 & 0.36 & 0.24 & 0.42 \\
 & \checkmark & 0.66 & 0.32 & 1.22 & 0.60 & 0.33 & 0.51 \\
\checkmark & \checkmark &  \textbf{0.43}& \textbf{0.15} &\textbf{0.48}& \textbf{0.29} & \textbf{0.21} & \textbf{0.31} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/tab4.tex <==
\begin{table}
\caption{Comparison of goal-oriented visual prompts based on different types of visual prompts on ETH/UCY datasets and FDE($\downarrow$) as the evaluation metric.}
\label{tab2}
{\setlength{\tabcolsep}{1.2pt}
\begin{tabular}{c|cccccc}
\toprule
 & \textbf{ETH} & \textbf{HOTEL} & \textbf{UNIV} & \textbf{ZARA1} & \textbf{ZARA2} & \textbf{AVG} \\
\midrule
ImageNet-1K~\cite{imagenet} & 0.44 & 0.18 & 0.49 & 0.30 & 0.22 & 0.33 \\
Remote-CLIP~\cite{remoteclip} & \textbf{0.41} & 0.17 & 0.49 & \textbf{0.28} & 0.22 & \textbf{0.31}  \\
CLIP~\cite{clip} & 0.43& \textbf{0.15} &\textbf{0.48}& 0.29 & \textbf{0.21} & \textbf{0.31} \\
\bottomrule
\end{tabular}
}
\end{table}
